Using a thousand optimization tasks to learn hyperparameter search strategies

We present TaskSet, a dataset of tasks for use in training and evaluating optimizers. TaskSet is unique in its size and diversity, containing over a thousand tasks ranging from image classification with fully connected or convolutional neural networks, to variational autoencoders, to non-volume preserving flows on a variety of datasets. As an example application of such a dataset we explore meta-learning an ordered list of hyperparameters to try sequentially. By learning this hyperparameter list from data generated using TaskSet we achieve large speedups in sample efficiency over random search. Next we use the diversity of the TaskSet and our method for learning hyperparameter lists to empirically explore the generalization of these lists to new optimization tasks in a variety of settings including ImageNet classification with Resnet50 and LM1B language modeling with transformers. As part of this work we have opensourced code for all tasks, as well as ~29 million training curves for these problems and the corresponding hyperparameters.

==> scrap.tex <==


One critical property of hand designed algorithms is there ability to generalize to new problems. Adam, for example, can be applied anywhere form text classification, to image modeling, to Atari. For a meta-learned algorithm to be useful, we would like a similar level of generalization.

The parameterizations of 

generalization to unseen and new tasks. Despite this goal, thereWhile there has been tremendous success in task specific domains, we are interested in building We are interested The study of data in meta-learning. In this work,

Data is a crucial component to all machine learning systems. The ability to train and test in a consistent environment, allows for easy comparison and have propelled sub fields such as computer vision and language.
The field of algorithm design, however, does not have this luxury. It is up to the researcher to design a test setup to demonstrate there algorithmic improvements.
Recently, researchers have been trying to shift algorithm design to learned algorithm design. Data is lacking however, making comparison hard.
To make matters worse, papers do not do throughough baseline evaluations making it unclear if the proposed method matters.

One active area of hand designing learning algorithms, and meta-learning learning algorithms is learned optimizers.

Benchmarks in optimization is 

Additionally these datasets are offen quite small, consisting of only a handful of problems.
This is natural as creating learning task is many times harder than labeling a supervised dataset.
In this work we introduce a meta-training set of tasks.

Hparam search hardly ever leverages experience of knowledge from other problems. Wastes compute. Notion of this grid is just bad.


Our task set is built from a mixture of different types of problems commonly seen in deep learning. We design it to be fast to execute, and capable of running on CPU.

With this task set, we probe two things: first, we explore baseline, hand designed optimizer performance. Second, we meta-learn an extremely simple learned optimizer consisting of finding a list of adam hyper parameters.



Existing work on optimizer design uses a small number of test functions, little understanding.

In this work we introduce a dataset of tasks for use in developing optimizers.

We then use this dataset and a primitive version of meta-learning based on random search to learn simple, yet practical learned optimizers.

Bridge gap between hand and meta-learned optimizers.

We propose a dataset of tasks used to not only probe optimizer performance but act as meta-training set for simple learned optimziers.

With this set of tasks designed, we shift to learning practical optimizers that perform well. we explore hyper parameters in common optimizer and build an approach based on meta-learning lists of hyper parameters for more effective search.

Not a benchmark per say, but a dataset. Much in the same way that solving MNIST cannot be used to say we have solved computer vision, this meta-training set will hopefully be a tool to help develop optimizers either by hand, or via meta-learning.

hparam lists / compute spent wasted on doing hparam search (with an estimate?)



\subsection{Experimental method and Data}
We run a bunch of junk. Then do analysis after the fact.

\section{Fixed hyperparameter and hyper parameter search.}
Default configuration is to use a fixed learning rate -- say the tf, pytorch or karpathy default.
One level up is to consider search spaces. Often practitioners just search learning rate.
One more level up searching more than one parameter.

We demonstrate this emperically.
Compare differnet baseline optimizers as a function of number of hparams tried.
Unsurprisingly, we find hparam selection is critical.

Single shot evaluation -- Hyperparameter free methods vs tuned baselines?
